An LLM's Attempts to Adapt to Diverse Software Engineers' Problem-Solving Styles: More Inclusive & Equitable?

Software engineers use code-fluent large language models (LLMs) to help explain unfamiliar code, yet LLM explanations are not adapted to engineers' diverse problem-solving needs. We prompted an LLM to adapt to five problem-solving style types from an inclusive design method, the Gender Inclusiveness Magnifier (GenderMag). We ran a user study with software engineers to examine the impact of explanation adaptations on software engineers' perceptions, both for explanations which matched and mismatched engineers' problem-solving styles. We found that explanations were more frequently beneficial when they matched problem-solving style, but not every matching adaptation was equally beneficial; in some instances, diverse engineers found as much (or more) benefit from mismatched adaptations. Through an equity and inclusivity lens, our work highlights the benefits of having an LLM adapt its explanations to match engineers' diverse problem-solving style values, the potential harms when matched adaptations were not perceived well by engineers, and a comparison of how matching and mismatching LLM adaptations impacted diverse engineers.

==> 0-TODO-list.tex <==
\tableofcontents

\begin{enumerate}

\item VOCAB
    \begin{enumerate}
    \item AAA: The official commands for llama-3's ``Tim''-like adaptation and ``Abi''-like adaptation are in the commands file.

    \item VOCAB: "perceptions" -> "ratings"

\item VOCAB: "Engineers" -> "THE engineers" when referring to your participants. Why: these are the actual participants, not a general class of people.

\item VOCAB: "Engineers’ responses" isn't great.  Why: responses are Things.  Reviewers don't really get excited about Things.  This is as boring as "The data showed that the engineers ate the rotten apples". \\
    If you can find a way to make the actors be The Engineers, reviewers will find the paper more enticing.  eg, "The engineers ate the rotten apples."

\item VOCAB: AAA: Software engineers is okay a few times (not every time), but call them ``engineers'' as a shorthand.
%MMB: I think "software engineers" should be "software developers" throughout.  That way we can use "developers" as a shorthand when needed. Which will work much better than "users".
% {\color{red}AAA: Not sure we can. We asked them to respond to their years of software engineering experience, not their years of dev experience. Unless we frame this as ``All engineers are devs''?}
% {\color{blue}MMB: ok, the shorthand can be ``engineers'' if that's the correct thing.}

\item VOCAB: MMB: the phrases "end user" and "end-user" shouldn't be in this paper (except in related work, perhaps).  Why: even when technically correct, it will confuse our readers.

\item VOCAB: MMB: for the same reasons as "end user", best to avoid the word "user". Instead, we can use "engineer" (see above).

\item VOCAB: MMB: "responses" -> "explanations". Why: the paper is about explaining, not responses generally.

%Dropping, because this is going to open us up to reviewers' wrath 
% \item VOCAB: "mental model" -> "theory of mind"
\item VOCAB: The term ``mental model'' shouldn't be in this paper. Why: It's not about mental models or theory of mind anymore, unless we inject it in there.

\item VOCAB the term "align" shouldn't be in this paper

\item VOCAB: Avoid saying something is inequitable for \textit{one} group. Equity is a comparison between \textit{two} groups.

\item VOCAB: We talk about more/less inclusivity and more/less equity, rather than support/undermine or help/harm.



\end{enumerate} %vocab
   
\item AUDITS
    \begin{enumerate}

    \item AUDIT If we refer to something in some other section anywhere in the paper, we have to make sure that that thing exists and is where we say it is.  
    \\ eg, "As we pointed out in the Introduction..." -- check, did we point that out in the intro? 
    \\ eg, "The Appendices include x" -- check, do they actually include x?

    \item AUDIT. MMB: none of the "For HAI Practitioners" phrasing was convincing, so please drop that terminoology.  eg, instead of "For HAI Practitioners, this suggests..." -> "This suggests..."

    \item AUDIT: Make sure we're no longer referring to the Quality factor. It didn't load, so we're gonna drop it. Max ratings is 15 (not 19).

    \item AUDIT: Do \textit{all} figures have the Utility factor? It's no longer Usefulness, is it? Triple check anyway.
 
    
    \end{enumerate} %audits

\item ORDER
    \begin{enumerate}

    \item *** Always list the problem-solving styles in the same order as the paper. (in tables, in text, in figures).
    \item Abi before Tim. Be consistent in all text, figures, tables, ... unless there's a really good reason to make an exception somewhere.

    \end{enumerate} %order 

\item FIGURES and TABLES

\item GRAMMAR and PUNCTUATION:
    \begin{enumerate}
    \item GRAMMAR: check demonstratives surrounding ``participants'' (who vs that)
    \item GRAMMAR: "i.e.," means "that is,".  "e.g.," means "for example, " -- it appears that they may both being used to try to say "for example".
    \item PUNCTUATION: Use M-dashes (like this: ---), not N-dashes (like this: --).  N-dashes belong ONLY in numeric ranges (like 3--16).\\
    \item PUNCTUATION: the periods are often messed up for our participant quotes. \\BAD: ``The birds are flying.'' (R94). \\BAD: ``The birds are flying.'' (R94) \\GOOD: ``The birds are flying'' (R94).
    \\BEST: I think its clearer and better with the Participant ID first, like this: \\(R94): ``The birds are flying.''\\

    \end{enumerate} %grammar and punctuation
    
    \item WRITING WELL
    \begin{enumerate}
   
    \item TOPIC SENTENCE: is the 1st sentence a good topic sentence?  \\
    GOOD: "To answer RQs 1 \& 2, we". \\
    BAD: "Figure 4a (top) shows..." (starts out well, but then:) "...that participants had a wide variety of responses." (Bad if the parag's point isn't going to be  "wide variety").
    \item WRITING NIT: ``Here are/There are'' is a particularly weak way of writing a sentence.  \\
    Bad: ``There are bad apples in this barrel.''  Good: ``This barrel has bad apples.''\\
    Bad: ``There were situations in which participants ate the bad apples anyway.'' \\ Good: ``In some situations, participants ate the bad apples anyway.''\\
    Bad: ``Here are the reasons they regretted eating them:''\\
    Good: ``They regretted eating them because:''
    \item WRITING NIT: ``Only'' goes as close as possible to the thing it's "ONLYing"!  (eg: "I only eat pears." BAD if you mean pears are the only thing you eat. GOOD if the only thing you do with pears is eat them.
    \item WRITING CONSIDERATION TO THE READER: If you must refer to a table in the appendix, say so. (e.g., instead of ``Table 8'', say ''Appendix Table 8'' or some such.)

    \end{enumerate} %writing rules

\item Spell check\\
\item Global search ``FIXME'' 
\item Global search "**"
\end{enumerate}


\clearpage


\setcounter{fixmeTotalCounter}{0}



==> doc/Z_old_04_3_rq_transparent.tex <==
\section{Engineers identifying adaptations: Who for and how?}
\label{subsubsec:result-mutualMM-human-to-ai}


\boldify{Here's what RQ-MutualMM (\humanToAI{}) part (a) asked, and Figure~\ref{fig:02_boreas_caelum_alignment_boxplot} shows that these participants succeeded for \textit{both} adaptations.}

% \topic{To answer \textbf{RQ-MutualMM (\humanToAI{})} to to empower diverse developers, part (a) asked whether and how developers could align their mental models with an LLM to deduce who it adapted its explanations for.}
\topic{Overall, participants succeeded at distinguishing between Llama-3-A's and Llama-3-T's adaptions.}
% Figure~\ref{fig:02_boreas_caelum_alignment_boxplot} shows that participants triumphed for \textit{both} adaptations.
Figure ~\ref{fig:02_boreas_caelum_alignment_boxplot} shows the boxplot of the aggregated ratings across all participants, when asked to identify if a particular LLM explanation was more ``Abi-like'' or more ``Tim-like.''
(Participants actually ranked each explanation per learning-style, but we've aggregated responses for analysis.)
% Recall from Section~\ref{subsubsec:adapting_LLMs} that \llamaTim{} tried to adapt for ``Tim''-like developers.
% Participants' average ratings of who they thought it was adapted for aligned (Figure~\ref{fig:02_boreas_caelum_alignment_boxplot}, top $\times$), trending towards the ``Tim''-like side.
% In fact, this was a statistically significant deviation from the midpoint, with a small \textit{practically} significant effect \tTestResult{2}{52}{2.1559}{.0357}{0.2961}\footnote{Cohen's d is a measure of practical effect size, where $d \in [0, 0.2)$ is no effect, $d \in [0.2, 0.5)$ is a small effect, $d \in [0.5, 0.8)$ is a medium effect, and $d \geq 0.8$ is a large effect, by convention~\cite{ramsey2012statistical}.};
For \llamaPersona{T}, we measured a small effect\footnote{Cohen's d is a measure of practical effect size, where $d \in [0, 0.2)$ is no effect, $d \in [0.2, 0.5)$ is a small effect, $d \in [0.5, 0.8)$ is a medium effect, and $d \geq 0.8$ is a large effect, by convention~\cite{ramsey2012statistical}.} \tTestResult{2}{52}{2.1559}{.0357}{0.2961}.
This meant that participants were more likely to say that \llamaPersona{T} was aligned with a ``Tim''-like developer than an ``Abi''-like one \odds{``Tim''}{1.304}.
% Participants were also successful in rating their alignment for
% \llamaAbi{}'s explanations;
For \llamaPersona{A}, we measured a medium effect \tTestResult{2}{52}{3.8077}{.0004}{.5230}.
% Figure~\ref{fig:02_boreas_caelum_alignment_boxplot} (bottom) reflects their success, showing participants' average more strongly leaned towards the ``Abi''-like side, a significant departure from the midpoint with a medium effect size \tTestResult{2}{52}{3.8077}{.0004}{.5230}.
Overall, participants were over 1.5 times more likely to correctly identify that these explanations were adapted for ``Abi''-like developers overall \odds{``Abi''}{1.789}.
These results suggest that participants \textit{could} correctly identify and align their mental models with the LLM's and deduced who the code explanations were adapted for.

\input{figures/02_boreas_caelum_alignment_boxplot}



% \boldify{We know this because participants rated both Boreas' and Caelum's output on an alignment scale, stating whether they thought the LLms were more aligned for the Tim-like or Abi-like problem-solving style value, and we centered these around zero (aligned to nobody)}

% \topic{These data were derived from participants' ratings of both Boreas and Caelum on a 7-point alignment scale on whether these models were better aligned for a ``Tim''-like or ``Abi''-like problem-solver.}
% As mentioned in Section~\ref{sec:methods}, participants had no knowledge of the specific values shown in Table~\ref{tab:01-GenderMag-Persona-Table} (e.g., comprehensive/selective information processing style or risk averse/tolerant).
% Instead, they were provided the more abstract definitions found on gendermag.org.
% For example, for information processing styles, participants were told that AI product users range from a ``burst-y'' (i.e., comprehensive) or ``incremental'' (i.e., selective) information processing style.
% These were the extreme end-points of the alignment scale that participants rated both Boreas and Caelum.

\boldify{Participants exhibited differing variances in their ratings between llama-3's Boreas and Caelum adaptations.
Llama-3's Boreas adaptation did not seem to do well for Learning Style, so only 36.36\% of participants correctly identified that it was aligned for ``Tim''. However, they thrived for Motivations!}

% \topic{This variability in participants' responses continued at the level of problem-solving style type (Table~\ref{tab:08_boreas_tim_alignment_counts}).}
\topic{Zooming in on specific problem-solving styles' ratings for \llamaPersona{T} shows that some of the LLM's problem-solving style adaptations were more easily identified than others.}
% This table shows participants' triumphs and trials with identifying the alignment for llama-3's Boreas adaptation.
Table~\ref{tab:08_boreas_tim_alignment_counts} shows how participants' rankings were distributed.
The right end of each row shows the proportion of participants who correctly rated that \llamaPersona{T} adapted for a ``Tim''-like user.
Participants' correct ratings showed a relatively wide spread (range: 32.73\%; sd = 12.177\%), suggesting that some adaptations from \llamaPersona{T} were more obvious than others to these participants.
% The table also suggests that \llamaTim{} struggled the most to adapt to the Learning Style type;
Notably, participants struggled to accurately identify the Llama-3-T's adaptations for the Learning Style type.
Only 40\% of participants correctly rated that this adaptation was for a more tinkering-oriented learner, which was the \textit{only} problem-solving style where participants thought that the adaptation was better suited for a process-oriented learner instead \odds{process}{1.5}.
% However, participants succeeded the most at identifying the alignment for \llamaTim{} regarding developers' motivations.
In contrast, 72.73\% of participants correctly identified that \llamaPersona{T} adapted to people with tech-oriented motivations \odds{tech}{2.667}.
These results suggest that for these five adaptations, there may need to be some adjustments to \textit{how} the system prompts are changed to help LLMs adapt their responses more clearly to empower people in deducing these ``Tim''-like alignments.

\input{tables/08_boreas_tim_alignment_counts}



%\input{tables/04_boreas_caelum_alignment}

\boldify{ Participants were far more consistent in correctly rating llama-3's Caelum adaptations across all five problem-solving style types (std. dev: 5.13\%). However, Learning Style \textit{and} information processing style were the most problematic.}

% \topic{Table~\ref{tab:09_caelum_abi_alignment_counts} shows that the significant difference in participants' average rating of \llamaAbi{} adaptation (Figure~\ref{fig:02_boreas_caelum_alignment_boxplot}) was due in part to their triumphs across \textit{all five} problem-solving styles.}
\topic{Unlike the ``Tim-like'' adaptations, participants were able to correctly identify ``Abi-like'' adaptations across all five problem-solving styles.}
In fact, the spread of participants' ratings for \llamaPersona{A} was about one \textit{third} of their spread for \llamaPersona{T} (range: 10\%; sd = 4.337\%).
\llamaPersona{A} was the weakest for both the learning style \textit{and} information processing style types, but still over half of the participants successfully identified both of these adaptations to process-oriented learners and comprehensive information processors \odds{process}{1.500}.
\DP{I made changes to the text in this section up to here. Mostly cutting things down and simplifying.}

\input{tables/09_caelum_abi_alignment_counts}


\boldify{So what trials did software engineers face when rating\llamaPersona{T} and \llamaPersona{A}? The most frequent (9 participants) was that they had flipped which was more rated for whom (Boreas $\implies$ Abi, Caelum $\implies$ Tim) }

\topic{The second part of \textbf{RQ-MutualMM (\humanToAI{})} asked what trials and triumphs developers faced when aligning their mental models with an LLMs'.}
Looking at participants' numeric ratings of each adaptation uncovered five categories of trials, where participants---1) found no adaptation in \textit{one}, 2) rated that the LLMs adapted to their \textit{opposite} value, 3) rated both as more ``Tim''-like (but one more so), 4) rated both as more ``Abi''-like (but one more so), and 5) rated both LLMs with the same alignment value.
The most frequently occurring of these categories was no detectable adaptation, 

\MMB{Vocab check: I think it's mutual ToM you want here, not mutual MMs...}


\boldify{The second-most frequent ( was the ``adapted to the opposite value'' trial, and participants had many reasons for thinking this}

where participants thought either \llamaPersona{T} was adapted for an ``Abi''-like developer and that \llamaPersona{A} was adapted for a ``Tim''-like developer.
In total, seven participants reversed who they thought \llamaPersona{T} and \llamaPersona{A} adapted for, and Table~\ref{**FIXME**} shows these participants' responses




\boldify{Engineers had diverse reasons for believing that certain alignments were more Abi-like or Tim-like, and here's how that contributed to **struggles**}

\boldify{These are an example of second-order mental models}

\FIXME{AAA}{Any further interpretation or drill-down can go here, but only what NEEDS to be said. If nothing interesting, say nothing.}



\clearpage



==> doc/Z_old_04_RQ_other.tex <==
\section{Results: **Other stuff that isn't the taxonomy**}

\FIXME{AAA}{I definitely want to talk about P18 here with the ``they got me'' comment.}

\FIXME{AAA}{Level 77 is a purely legacy COBOL level. It won't feature in newer code.}

\subsection{``Why hasn't it described that?''---What participants wanted explained}


\boldify{Keywords}

\textbf{Note:} does this cluster by any of the problem-solving styles?

\FIXME{AAA}{Thoughts:

Do we have cross-cutting results for problem-solving style X programming expertise? For example, is there a model where the adaptations to information processing style appear also in the beginner/expert programmer?}


\FIXME{AAA}{We have other problem-solving styles interfering with the ones it's supposed to be adapting to (think P02).

We also have people saying that when the LLMs try to adapt by bringing up information about what it thinks it knows about people, they view it as extraneous information.

Another observation is that some output adaptations added extra phrases, trying to be supportive for risk-averse or lower self-efficacy.
However, task-oriented motivations took over here;
they wanted to get to the meat without the fluff.

I've seen two people with lower self-efficacy people asking for attribution like links for some of the questions at the end.
They're suggesting that attribution is an adaptation that would suit their needs.}


\FIXME{AAA}{I think that there's a structure we may want to consider for this section, where we look at what they liked when they liked the LLM they were ``supposed to'' (i.e., alignment) and when they didn't like what they were supposed to (i.e., misalignment).

I'm thinking about this because I've noticed that some risk-averse people or comprehensive people sometimes don't like Caelum. SImilarly, sometimes they really like Boreas.

These are unexpected outcomes.}

\subsection{Links, References, and Documentation---The tie to self-efficacy}

==> doc/Z_old_04_RQ_taxonomy.tex <==
\section{Results: Taxonomies of Helpful/Problematic Adaptations}
\label{sec:results}
\FIXME{AAA}{Show, don't tell}

\subsection{``I would love for all of this to have never been printed…''---Adapt, don't tell!}

\boldify{One of the most obvious ways that LLMs could adapt their output would be to just \textit{tell} someone about their problem-solving style values.}

\boldify{This was one of the adaptation patterns that Llama-3 adopted, and it did so at least once for **\textit{every}** problem-solving style value in at least one of the problems (Table~\ref{**FIXME})}

\FIXME{AAA}{There may be something about providing the division headers. Some people seem to appreciate the clarity that it brings and the organizational structure, whereas others like them because it confirms hypotheses that they have.}

\boldify{}


==> doc/z-leftovers.tex <==

AAA - These are the two research questions that can come after an IUI paper.

\item \textbf{RQ-Helpful-Taxonomy:} What aspects of the large language models' outputs and adaptations do software developers find helpful for their understanding of COBOL programs?

    % \begin{enumerate}
    %     \item \textit{Measure}: Helpful information
    % \end{enumerate}

    \item \textbf{RQ-Problematic-Taxonomy:} What aspects of the large language models' outputs and adaptations do software developers find problematic for their understanding of COBOL programs?

    % \begin{enumerate}
    %     \item \textit{Measure}: Problematic information
    % \end{enumerate}




    
\quoteWithLLM{04}{Mot}{Tech}{Match}{I'm saying uncertain because [\llamaWithVal{TimBlue}{Mot}{Tech}] missed out key information about certain areas of the codes...% 
%such as like not talking about `Display Error', not talking about the END-EVALUATE, kind of skipping over what these sections [highlighted the WORKING-STORAGE SECTION and PROCEDURE DIVISION sections] all are.
}

\quoteWithLLM{04}{Mot}{Tech}{Match}{I felt productive... not really. 
% At least the other two [LLM explanations] had some sort of shape to them that was helpful, like [unadapted Llama-3] was helpful with actually reading through the code, but [\llamaWithVal{AbiOrange}{Mot}{Task}] had better structure.
[\llamaWithVal{TimBlue}{Mot}{Tech}], I feel, was just too chatty at the start and then didn't really understand what was happening.}





When talking about the overly friendly greeting








When responding to Mental Demand in Cognitive :

\quoteWithLLM{04}{Mot}{Tech}{Match}{I think it was easier to understand, but it wasn't good enough at explaining it.}




\boldify{The answer to RQ-Unadapted-LLM-Equity was that it depended on the treatment; you gotta look at the five independently.}

% \topic{Throughout this section, we saw that the answer to \textbf{RQ-Unadapted-LLM-Equity} was nuanced, depending on the problem-solving style type at hand.}
% For example, Section~\ref{subsec:two_inclusivities_resolves_inequity} highlighted that the \personaVal{AbiOrange}{process-oriented} learners were inequitably disadvantaged by the unadapted llama-3 explanations more frequently than their \personaVal{TimBlue}{tinkering-oriented} peers.
% However, Section~\ref{subsubsec:one_inclusivity_resolves_inequity} highlighted skewed inequity disadvantages for engineers with \personaVal{AbiOrange}{lower} self-efficacies and a more \personaVal{TimBlue}{risk-tolerant} attitude.
% For AI practitioners, these results suggest that finding out who are disadvantaged when LLMs do not adapt their explanations to suit diverse engineers requires a holistic view of all five styles in this paper. 

% \boldify{Additionally, for RQ-Adapted-``to me'' showed that generally, adapting LLMs to match engineers worked awesome! Diverse learning styles, self-efficacies, and risk attitudes got exactly what they needed to close inequities. }

% \topic{More often than not, the answer to both the inclusion and equity parts of \textbf{RQ-Adaptations-Match-Engineers} was positive.}
% When llama-3 adapted its explanations to match the learning style, self-efficacy, and risk values of diverse engineers, the engineers whose perceptions were inequitably disadvantaged by the \textit{un}adapted llama-3 received the support they needed to narrow inequities.
% Sometimes, both values needed the support in order to close these inequities (Section~\ref{subsec:two_inclusivities_resolves_inequity}), and other times, the support that one value received was sufficient to close inequities (Section~\ref{subsubsec:one_inclusivity_resolves_inequity}).
% Additionally, although the GenderMag literature has repeatedly shown that the more ``Abi''-like problem-solvers are disparately impacted by technology (e.g.,~\cite{anderson-diversity-2024,beckwith2004gender,beckwith2006tinkering}), ``Tim''-like problem-solvers may also need support from inclusively designed technologies.
% These results re-affirm this finding for the \HAI{} community, since both ``Abi''-like \textit{and} ``Tim''-like engineers found themselves inequitably disadvantaged by treatment. 





\AAA{I'm putting this here for now. 1) Space. 2) We don't talk about IP in the previous section.}

\subsection{Information Processing Style Mismatches Produced More Support \textit{and} Undermined Less?
\draftStatus{AAA}{2}}

\boldify{For diverse information processing styles, the answer to RQ-Adaptations-Mismatch-Engineers was that \textit{mismatching} was both more supportive and less harmful for both comprehensive...}

\topic{A second phenomenon arose for engineers' diverse information processing styles, showing the \textit{mis}matching adaptation as helping \textit{more} and harming \textit{less}.}
The left side of Figure~\ref{fig:02_info_inclusion_not_for_me} contrasts how \llamaWithVal{AbiOrange}{InfoProc}{Comprehensive} (top) and \llamaWithVal{TimBlue}{InfoProc}{Selective} (bottom) inclusively supported \personaVal{AbiOrange}{comprehensive} information processors.
These engineers actually received two inclusivity boosts to their suspicions of llama-3 (Trust) and effort (Cognitive Load).
Additionally, they were undermined less frequently by \llamaWithVal{white}{InfoProc}{Selective} (3/19) than they were by llama-3-InfoProc-Comprehensive (12/19).


\input{figures/dv_inclusion_not_for_me_figures/02_info_inclusion_not_for_me}

\boldify{...and selective information processors too!}

\topic{\personaVal{TimBlue}{Selective} information processors also derived more benefit from the \llamaWithVal{AbiOrange}{InfoProc}{Comprehensive} explanations.}
For example, Section~\ref{subsec:exclusive_inequitable} highlighted that selective information processors received \textit{zero} inclusivity benefits from \llamaWithVal{white}{InfoProc}{Selective}, yet engineers' reported that they had incurred more mental demand and effort for lower performances.
However, 

% \AAA{P28 saw \llamaWithVal{white}{InfoProc}{Comprehensive} explain the RPS program. 
% They initially highlighted the first two lines as helpful, saying ``These are helpful'' and then highlighted the 7 lines under there, saying ``these are obsolete. They're all the same, so there is no need to explain all the others. I think it's pretty obvious.''}

% \quoteWithLLM{28}{InfoProc}{Selective}{Mismatch}{I thought that [these 7 lines] were obsolete, but now I see that there's more information in here to understand the actual program. I was too quick here to judge.}

\boldify{Some of the selective information processors drew direct comparisons between the adaptations, commenting on how they preferred the amount of information that llama-3-InfoProc-Comprehensive provided...}

\topic{Some engineers with a more \personaVal{TimBlue}{selective} information processing style shed light on why they received more inclusivity benefits from \llamaWithVal{white}{InfoProc}{Comprehensive} through direct comparisons.}
For example, two of the engineers pointed out that the mismatching adaptation had provided additional information by explaining all of the program logic: 
\quoteWithLLM{TimBlue}{28}{InfoProc}{Selective}{AbiOrange}{Mismatch}{I felt like [\llamaWithVal{white}{InfoProc}{Comprehensive}] was better in terms of like describing the relevant information that I was lacking in order to understand the program.}
%
or by elaborating on some keywords in the Infinite Loop program, such as PERFORM, VARYING, UNTIL, and AFTER:
%
\quoteWithLLM{TimBlue}{40}{InfoProc}{Selective}{AbiOrange}{Mismatch}{I feel that [\llamaWithVal{white}{InfoProc}{Comprehensive}] worked better for me [than Llama-3-InfoProc-Selective] because it picked out all of these keywords that are there in COBOL and it explained those keywords...}

\boldify{Since two selective information processors mentioned the amount of informaiton presented, one possibility is that Llama-3-InfoProc-Selective's attempt to adapt had erred on the side of caution, not wanting to overwhelm their selective user.}

\topic{Two selective information processors mentioned that they preferred having \textit{more} information from Llama-3-InfoProc-Comprehensive.}
The literature has found that in information rich environments, such as in programming, selective information processors approaches are more incremental;
they usually delve into the first promising option, pursuing that option as far as they can.
If that option does not work out, they back out and gather a bit more information until they discover another option to try.
One possibility is that while trying to adapt for engineers' selective information processing styles, llama-3 may have cut back on the amount of information it displayed 

% \boldify{... and even the format of information.}

% \topic{Both participants also mentioned information presentation made a difference for them.}
% For example, P28 commented on the structural differences of similar information between Llama-3-InfoProc-Selective and LLama-3-InfoProc-Comprehensive:

% \quoteWithLLM{28}{InfoProc}{Selective}{Mismatch}{I felt like [\llamaWithVal{white}{InfoProc}{Comprehensive}'s] structure itself of having a header and then the content is better for me, easier for me to digest, rather than having <<header>> : <<content>>.}

% \FIXME{AAA}{Note: The above quote, the participant literally said ``header colon content'' and highlighted an example.}

% They were referring to the fact that \llamaWithVal{white}{InfoProc}{Selective}'s explanation placed 

% \llmSnippet{\llamaWithVal{TimBlue}{InfoProc}{Selective}}
% {Infinite Loop}
% {**DATA DIVISION**: This section defines the data structures used in the program...}



% whereas \llamaWithVal{white}{InfoProc}{Comprehensive}'s explanation displayed broke them up with line breaks:

% \llmSnippet{\llamaWithVal{AbiOrange}{InfoProc}{Comprehensive}}
% {Rock-Paper-Scissors}
% { **Data Division:**
%     \\
%     In this section, two working storage variables are defined...
% }


% \quoteWithLLM{40}{InfoProc}{Selective}{Mismatch}{[\llamaWithVal{white}{InfoProc}{Selective}]'s presentation format is also not that concise compared to [\llamaWithVal{white}{InfoProc}{Comprehensive}]... [\llamaWithVal{white}{InfoProc}{Selective}] is just making me read more and more.}




\boldify{Although the mismatched adaptations did provide some utility, it does not mean that they were a panacea. For example, some of the selective information processors commented on how they felt forced to consume a \textit{whole} explanation.}

\topic{Although \llamaWithVal{white}{InfoProc}{Comprehensive} provided selective information processors with some inclusivity benefits, it was not a silver bullet for their information processing needs.}
For example, P40 provided two potential solutions to adjust the explanation's formatting to support their information processing endeavors.
Their first suggestion aimed to help their ability to search for relevant information in the explanation:

\quoteWithLLM{TimBlue}{40}{InfoProc}{Selective}{AbiOrange}{Mismatch}{If [the explanation] formatting was a little different, something like bold titles, keywords standing out, it could have helped me a bit more to quickly identify the keywords while looking at the response, instead of having to read through the whole thing.}
%
While explaining that they had felt mentally demanded, P40 expanded brought up their how their proposed solution would empower them to quickly find promising pieces of information to tie to the COBOL program:
%
\quoteWithLLM{TimBlue}{40}{InfoProc}{Selective}{AbiOrange}{Mismatch}{[The explanation] was a little mentally demanding for sure, because I had to read through the whole thing, and it took up a good five minutes of my time. 
I want things to stand out and just use the keywords and then link the sentences together.}

% P40's second suggestion 



% \quoteWithLLM{40}{InfoProc}{Selective}{Mismatch}{If this description [highlights the summary sentence] was better, like in a paragraph format and then it was broken down so that would also kind of give me a summary of everything and then I could look into it if I wanted to. I'd just pick out the things that I wanted to.}

==> figures/01-Programming-Methodology-Overview.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.5\linewidth]{assets/Figure-01-Programming-Methodology-Overview.pdf}
    \caption{The methodology to answer \textbf{RQ-LLM-Adapts}.
    For six LLMs, we provided two inputs---a user profile reflecting two dimensions of user diversity and a query to explain three COBOL programs.
    If LLMs adapted their outputs, were their query responses more inclusive, catering to their end user's diverse needs? \DP{Change "User Profile" to "Control or Facet-specific System Prompt" and "User Query" to "Request for Code Explanation" }}
    \label{fig:01-Programming-Methodology-Overview}
\end{figure}

==> figures/02_boreas_caelum_alignment_boxplot.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.55\linewidth]{assets/boreas_caelum_alignment_boxplot.pdf}
    \caption{Participants' alignment ratings for the five \colorboxBackgroundForegroundText{TimBlue}{black}{\llamaPersona{T}} (top) and five \colorboxBackgroundForegroundText{AbiOrange}{black}{\llamaPersona{A}} (bottom) from most ``Abi''-like (left) to most ``Tim''-like (right).
    From the midpoint (value of 0), participants' average rating of both \llamaPersona{T} (positive values) and \llamaPersona{A} (negative values) were aligned to their corresponding problem-solving styles.}
    \DP{I rewrote the text above assuming that the figure will be simplified as MMB suggested.}

    % \FIXME{MMB}{(1)need to say what the orange bar is and what the blue bar is.\\
    % AAA---Used colour binding in the first sentence.\\
    % (2) AAA---Used the exact same RGBs we used for MSR paper.  \\
    % MMB: Still looks pink-ish to me here.  Can you try to make it orange-er??}
    \label{fig:02_boreas_caelum_alignment_boxplot}
\end{figure}

==> figures/04_llama_3_baseline_tim_favor.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{assets/Llama_3_baseline_tim_favor.pdf}
    \caption{The number of dependent variables (y-axis) by treatment (x-axis) where either the \colorboxBackgroundForegroundText{TimBlue}{black}{the ``Tim''-like} or \colorboxBackgroundForegroundText{AbiOrange}{black}{the ``Abi''-like} participants' average was 10\% greater than their counterparts'.
    For three treatments (left), \llamaNone{} favored ``Tim''-like participants more often.
    For the last two, it favored ``Abi''-like participants more.
    %, suggesting room for improvement for \textit{both}.
    }
    \MMB{It suggests something more interesting than "room for improvement" (so I commented that out.) To me, seems like we can write something interesting. eg: The risk facet results favoring Abi, could be the perfect thing to do -- after all, the risk-tolerant might not even ask an LLM for an explanation. On the other hand, the favoring high-SE is a real problem.  I think there's interesting stuff to be said for the other facets too.  Maybe in results, or maybe in discussion.}
    \label{fig:04_llama_3_baseline_tim_favor}
\end{figure}

==> figures/05_DV_Distance_Example.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{assets/DV_Distance_Example.pdf}
    \caption{The averages (diamonds) for \colorboxBackgroundForegroundText{AbiOrange}{black}{process-oriented} and \colorboxBackgroundForegroundText{TimBlue}{black}{tinkering-oriented} learners for the Feelings factor's five dependent variables (Table~\ref{tab:10_llm_dv_table}).
    Small sample sizes (n = 11) make statistical tests less meaningful, but 10\% gaps between averages reveal potential differences.
    We include distances between means greater than 10\% (red) as potential inclusivity differences.
    However, we exclude distances less than 10\% (black), due to similar perceptions for diverse engineers.
    For this factor, three of the five dependent variables were included.}
    \label{fig:05_DV_Distance_Example}
\end{figure}

==> figures/06_equity_all_prob_solve_styles.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.8\linewidth]{assets/Equity_all_prob_solve_styles.pdf}
    \caption{For each of the five problem-solving styles (plots), the percentage (y-axes) of \textit{who} benefited from 10\% inequities (left-most bar)  }
    \label{fig:enter-label}
\end{figure}

==> figures/07_radar_plots_probsolve_style_adapt.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{assets/07_radar_plots_probsolve_style_adapt.png}
    \caption{Radar plots for hypothetical inclusive support across problem-solving styles (vertices).
    Notice the decrease in support as an LLM adapts from one problem-solving style (left) to five (right), since LLMs have finite ``attention'' to adapt.}
    \label{fig:07_radar_plots_probsolve_style_adapt}
\end{figure}

==> figures/dv_equity_figures/01_learn_unadapted_equity.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.62\linewidth]{assets/dv_equity_assets/unadapted_equity_assets/learn_unadapted_equity.pdf}
    \caption{Unadapted LLM: The number of dependent variables (x-axis) where the \personaVal{AbiOrange}{process-oriented} %($\leftarrow$) 
    or \personaVal{TimBlue}{tinkering-oriented} %($\rightarrow$) 
    learners were inequitably advantaged across the five question categories (y-axis) from Table~\ref{tab:10_llm_dv_table}.
    Notice that process-oriented learners had fewer advantages, suggesting that tinkering-oriented learners were ``favored'' by the unadapted llama-3.
    Note: One box = One dependent variable in each category.}
    \label{fig:01_learn_unadapted_equity}
    % \MMB{Figure looks weird -- why don't the lines line up?  It's just counting variables, so shouldn't each little box be exactly one DV, and shouldn't the boxes be the same size?  Really confusing.}
    % \MMB{And just BTW, you don't need the legend, the caption already says what orange and blue mean.}

    % \AAA{Categories have either 5, 3, or 4 variables in them. So for the Feelings line, we see Abi is disadvantaged 3/5 times. For Trust, 3/3. If we had each box be the same size, then the Trust looks equally as bad (whereas it's worse) than the Feelings.}
    % \MMB{Then what 1 box equals needs to be clarified in the caption.  Or perhaps no boxes at all, and just make the numbers be a percent of what's possible.  (100\% or 33\% or whatever).}

\end{figure}

==> figures/dv_equity_figures/03_se_risk_unadapted_equity.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{cp{0.01\linewidth}c}
    % \multicolumn{3}{c}{Equity Disadvantages for Unadapted Llama-3}\\
    Computer Self-efficacy & & Attitudes Toward Risk\\
     \includegraphics[width =.47\linewidth]{assets/dv_equity_assets/unadapted_equity_assets/se_unadapted_equity.pdf} &
     &
     \includegraphics[width=.47\linewidth]{assets/dv_equity_assets/unadapted_equity_assets/risk_unadapted_equity.pdf}   
    \end{tabular}
    \caption{The inequity graphs for computer self-efficacy (left) and attitudes toward risk (right) when llama-3 was unadapted.
    Notice that for computer self-efficacy, the \personaVal{AbiOrange}{lower} self-efficacy ($\leftarrow$) participants were inequitably disadvantaged, relative to the \personaVal{TimBlue}{higher} self-efficacy ($\rightarrow$).
    Alternatively, for attitudes toward risk, the \personaVal{AbiOrange}{risk-averse} ($\leftarrow$) were inequitably advantaged, relative to the \personaVal{TimBlue}{risk-tolerant} ($\rightarrow$).
    }
    \label{fig:03_se_risk_unadapted_equity}
\end{figure}

==> figures/dv_equity_figures/04_se_equity_changes.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{cc}
    % \multicolumn{3}{c}{Equity Disadvantages for Unadapted Llama-3}\\
    Unadapted LLM Inequity & Adapted LLM (same value) Inequity \\
     \includegraphics[width =.48\linewidth]{assets/dv_equity_assets/unadapted_equity_assets/se_unadapted_equity.pdf} &
     \includegraphics[width=.48\linewidth]{assets/dv_equity_assets/adapted_for_me_equity_assets/se_adapted_equity_for_me.pdf}   
    \end{tabular}
    \caption{The number of inequities for the unadapted LLM (left) and the self-efficacy adapted LLMs (right) between engineers with \personaVal{AbiOrange}{lower} and \personaVal{TimBlue}{higher} self-efficacy values.
    For the unadapted LLM, \textit{all} of the disadvantages went against the \personaVal{white}{lower} self-efficacy engineers.
    However, \llamaWithVal{AbiOrange}{SelfEff}{Lower} increased inclusivity so frequently (Figure~\ref{fig:02_se_inclusion_for_me}) that inequities were almost erased.
    \DP{Same comments about titles and axis}}
    \label{fig:04_se_equity_changes}
\end{figure}

==> figures/dv_equity_figures/06_ip_mot_adapted_equity_for_me.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{cp{0.01\linewidth}c}
    % \multicolumn{3}{c}{Equity Disadvantages for Unadapted Llama-3}\\
    Information Processing Style & & Motivations\\
     \includegraphics[width =.47\linewidth]{assets/dv_equity_assets/adapted_for_me_equity_assets/ip_adapted_equity_for_me.pdf} &
     &
     \includegraphics[width=.47\linewidth]{assets/dv_equity_assets/adapted_for_me_equity_assets/mot_adapted_equity_for_me.pdf}   
    \end{tabular}
    \caption{The inequity graphs for information processing style (left) and motivations (right) when llama-3 was unadapted.
    Notice that overall, the number of inequities were not as frequent as Section~\ref{subsec:two_inclusivities_resolves_inequity} (i.e., $< 10$) and not as skewed as Section~\ref{subsubsec:one_inclusivity_resolves_inequity}.
    }
    \label{fig:06_ip_mot_adapted_equity_for_me}
\end{figure}

==> figures/dv_inclusion_not_for_me_figures/02_info_inclusion_not_for_me.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{cp{0.01\linewidth}c}
    % \multicolumn{3}{c}{Equity Disadvantages for Unadapted Llama-3}\\
    Comprehensive Information Processors & & Selective Information Processors \\
     \includegraphics[width =.15\linewidth]{assets/dv_inclusion_assets/inclusion_for_me_assets/ip_comp_inclusion_for_me.png} &
     &
     \includegraphics[width=.15\linewidth]{assets/dv_inclusion_assets/inclusion_for_me_assets/ip_sel_inclusion_for_me.png}  \\
     %
     %
     %
     %
     \includegraphics[width =.47\linewidth]{assets/dv_inclusion_assets/inclusion_not_for_me_assets/ip_comp_inclusion_not_for_me.png} &
     &
     \includegraphics[width=.47\linewidth]{assets/dv_inclusion_assets/inclusion_not_for_me_assets/ip_sel_inclusion_not_for_me.png}   
    \end{tabular}
    \caption{How supported ($\rightarrow$) and undermined ($\leftarrow$) perception inclusivity was for \personaVal{AbiOrange}{comprehensive} (left) and \personaVal{TimBlue}{selective} (right) information processors between the adaptations which matched their styles (top row, see Section~\ref{subsec:exclusive_inequitable}) and did \textit{not} match them (bottom row).
    When the adaptations did not match, both information processing styles were better helped \textit{and} less harmed.
    }
    \label{fig:02_info_inclusion_not_for_me}
\end{figure}

==> figures/dv_inclusion_not_for_me_figures/03_mot_inclusion_not_for_me.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{cp{0.01\linewidth}c}
     \includegraphics[width =.47\linewidth]{assets/dv_inclusion_assets/inclusion_not_for_me_assets/mot_task_inclusion_not_for_me.png} &
     &
     \includegraphics[width=.47\linewidth]{assets/dv_inclusion_assets/inclusion_not_for_me_assets/mot_tech_inclusion_not_for_me.png}   
    \end{tabular}
    \caption{\fixfixfix{Usefulness $\rightarrow$ Utility.} How supported ($\rightarrow$) and undermined ($\leftarrow$) perception inclusivity was for engineers with \personaVal{AbiOrange}{task-oriented} (left) and \personaVal{TimBlue}{tech-oriented} (right) motivations between adaptations that matched their motivations (top row, see Section~\ref{subsec:exclusive_inequitable}) and  those which did \textit{not} (bottom row).
    Unexpectedly, when the adaptations did not match, both information processing style groups were more supported \textit{and} less undermined.
    \DP{titles and axes? Also, little, itty, bitty figures.}}
    \label{fig:03_mot_inclusion_not_for_me}
\end{figure}

==> tables/03-Info-Proc-Questions.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{|p{\linewidth}|}
    \hline
    \small
    \textbf{Agreement Questions}\\
    \textbf{1.} ``\textit{I want to get things right the first time, so before I decide how to take action, I gather as much information as I can.}''\\
    \textbf{2.} ``\textit{I always do extensive research and comparison shopping before making important purchases.}''\\
    \textbf{3.} ``\textit{When a decision needs to be made, it is important to me to gather relevant details before deciding, in order to be sure of the direction we are heading.}''\\
    \\
    \textbf{Alignment Question}\\
    ``\textit{When I’m using technology, I collect the minimal amount of relevant information needed to take action. 
    I act quickly; knowing I can come back later and resolve things if I need to.}''\\
    \multicolumn{1}{|c|}{\textbf{OR}}\\
    ``\textit{When I’m using technology, I opt to collect as much information as I can before taking action. 
    For me, full understanding of a situation is more important than speed.}''\\
    \hline
    \end{tabular}
    \caption{\textbf{Top:} Three agreement questions about information processing style~\cite{anderson-diversity-2024}.
    \textbf{Bottom:} Alignment statements, one for each end of the information processing style spectrum.
    Those who have a more \textit{selective} information processing style are more likely to disagree with the agreements and align with the first alignment statement.
    Alternatively, those with a more \textit{comprehensive} style are more likely to do the opposite.}
    \label{tab:03-Info-Proc-Questions}
\end{table}

==> tables/04_boreas_caelum_alignment.tex <==
\begin{table}[h]
    \centering
    \includegraphics[width =\linewidth]{assets/participants_alignment_agreement_by_style.pdf}
    \caption{\textbf{(Left)} The count of responses for llama-3's Boreas adaptation being more ``Tim''-like or not.
    Notice the variety in participants' success rates, ranging from a minimum of 36.36\% (Learning Style) to a maximum of 72.73\% (Motivations).\\
    \textbf{(Right)} The count of responses for llama-3's Caelum adaptation being more ``Abi''-like or not.
    Notice that participants were far more consistently successful;
    the minimum was 54.55\% (Learning Style) to 66.67\% (Self-Efficacy and Attitudes Toward Risk jointly).
    }
    \FIXME{AAA}{Put the number above the columns, so people know what the numbers actually mean.}
    \label{tab:04_boreas_caelum_alignment}
\end{table}

==> tables/07_participant_prob_solve_agreement.tex <==
\begin{table}[h]
    \centering
    \includegraphics[width = 0.75\linewidth]{assets/partiticipant_prob_solve_agreement.pdf}
    \caption{Participants' agreement responses to their problem-solving style type classification.
    85\% of participants agreed (i.e., answered with 5, 6, or 7) with their GenderMag problem-solving style classification.
    }
    \label{tab:07_participant_prob_solve_agreement}
\end{table}

==> tables/08_boreas_tim_alignment_counts.tex <==
\begin{table}[h]
    \centering
    \includegraphics[width = 0.8\linewidth]{assets/boreas_tim_alignment_counts.pdf}
    \caption{Count of participants who agreed (right) or disagreed (left) that \llamaPersona{T} adapted for a ``Tim''-like developer.
    Although responses cluster towards the right (i.e., the amount of red), the largest value exists in the \textit{left} side, where most participants in the learning style treatment thought \llamaPersona{T} was for an ``Abi''-like process-oriented learner.}
    %Agreement, not correctness
    \label{tab:08_boreas_tim_alignment_counts}
\end{table}

==> tables/09_caelum_abi_alignment_counts.tex <==
\begin{table}[h]
    \centering
    \includegraphics[width = 0.8\linewidth]{assets/caelum_abi_alignment_counts.pdf}
    \caption{Count of participants who rated whether \llamaPersona{A} was more adapted for an ``Abi''-like developer (right) or not (left).
    Although responses cluster towards the right (i.e., the amount of red), the largest value exists in the \textit{left} side, where most participants in the learning style treatment thought \llamaPersona{T} was for an ``Abi''-like process-oriented learner.}
    \label{tab:09_caelum_abi_alignment_counts}
\end{table}

==> tables/11_inclusion_match_mismatch_learning.tex <==
\begin{wraptable}{o}{0.4\linewidth}
    \centering
    \includegraphics[width = \linewidth]{assets/dv_inclusion_assets/inclusion_matched_mismatched_tables/learn_matched_mismatched_inclusion.png}
    \caption{The number of differences for supported (top row) and undermined (bottom row) perceptions between the two adaptations for engineers' learning styles.
    The \personaVal{AbiOrange}{process-oriented} learners lost support for 12 perceptions with \llamaWithVal{TimBlue}{Learn}{Tinker}.}
    \label{tab:11_inclusion_match_mismatch_learning}
\end{wraptable}
